SCALER: Breaking the Latent Scaling Bottleneck via Single-Pass Context-Anchored Latent Visual Reasoning

Longer chains of thought substantially improve language reasoning on complex problems, inspiring efforts to scale visual reasoning via continuous latents. However, evaluating visual latent reasoning across complexity and sequence length reveals a fundamental **Latent Scaling Bottleneck**: existing methods yield modest gains only within short budgets ($\leq 30$ tokens) on simple tasks, yet stagnate or *degrade* on harder tasks and longer chains. Controlled diagnostics trace this bottleneck to two root causes. First, **Latent Representation Saturation** under autoregressive conditioning causes step-wise cosine novelty to decay exponentially and saturate after $\sim 30$ steps. Second, **Over-Compressed Supervision Targets** from heavily pooled ($\geq 128\times$) image embeddings lose fine-grained spatial structure and act like meaningless padding. We propose **SCALER** (**S**ingle-Pass **C**ontext-**A**nchored **L**at**e**nt Visual **R**easoning), whose lightweight *detransformer* synthesizes spatially aligned auxiliary tokens from full-sequence hidden states *in a single forward pass*, anchoring each token to the original visual space. Coupled with three-stage SFT and **ALPO** (**A**uxiliary **L**atent **P**olicy **O**ptimization) for differentiable RL, SCALER extends effective latent length by over $30\times$, achieves state-of-the-art open-source accuracy (e.g., **57.84%** on MME-RealWorld-Lite, +12.09% over backbone, +10.47% over GPT-6-luna), with strong OOD generalization. Our project page: [https://bonjour-codedev.github.io/SCALER/](https://bonjour-codedev.github.io/SCALER/).

==> xref_main.tex <==
%Generated labels from main.tex; no manuscript content.
\SCOLARExternalLabel{fig:confusion_matrix}{{1}{1}{\textbf {The Latent Scaling Bottleneck Across Task Complexity (C1--C5) and Latent Token Budgets ($K \in [0, 1000]$).} Accuracy (\%) across five pooled benchmarks stratified into five complexity levels. Existing methods ((a) Monet, (b) LVR, (c) LASER, and (d) UniVLR) only exhibit positive length scaling in the shallow lower-left regime ($K \leq 30$, low complexity C1--C2), but stagnate or degrade in the upper-right regime of higher task complexity (C3--C5) and longer sequences ($K \geq 100$). In contrast, (e) \textbf {SCALER} sustains positive scaling across long latent budgets and achieves substantial gains on high-complexity tasks (C4--C5).\relax }{figure.caption.1}{main.pdf}}
\SCOLARExternalLabel{fig:confusion_matrix@cref}{{[figure][1][]1}{[1][1][]1}{}{}{main.pdf}}
\SCOLARExternalLabel{fig:motivation}{{2}{2}{\textbf {Root Cause Diagnosis and Our Single-Pass Context-Anchored Solution.} \textbf {Left:} Paradigm comparison. In conventional autoregressive latent reasoning, latent variable $L_n$ depends recursively on $L_{n-1}$, causing visual semantics to decay and representations to saturate (\textbf {Accuracy $\downarrow $}). Interleaved latent reasoning (ILVR) inserts short local latent spans between text tokens but lacks global high-resolution visual grounding. In \textbf {SCALER}, each auxiliary token independently anchors to the original visual semantic space in a single forward pass, preventing information decay (\textbf {Accuracy $\uparrow $}). \textbf {Right (a):} Latent length scaling on MME-RealWorld-Lite (scatter points, $\log _{10}$-length local quadratic fits, and 95\% bootstrap bands): SCALER recovers from moderate-pooling dips to peak at full length, whereas Monet and UniVLR plateau and degrade. \textbf {Right (b):} Step-wise cosine novelty on MME-RealWorld-Lite across 1K tokens: SCALER sustains high novelty ($10^{-1}\text {--}10^{0}$) throughout the sequence, whereas Monet and UniVLR decay exponentially to $10^{-3}\text {--}10^{-4}$ after $t \approx 30$.\relax }{figure.caption.2}{main.pdf}}
\SCOLARExternalLabel{fig:motivation@cref}{{[figure][2][]2}{[1][1][]2}{}{}{main.pdf}}
\SCOLARExternalLabel{fig:method}{{3}{3}{\textbf {Overview of the SCALER Inference Pipeline.} \textbf {Left:} Three-stage inference flow: (1)~\emph {Phase-1 Generate}: the LLM backbone processes text tokens and visual tokens $V$ until autonomously emitting the \texttt {<auxiliary>} trigger; (2)~\emph {Detransformer (Think Visually)}: full-sequence hidden states $H$ are mapped by $D_\phi $ in a single forward pass to visual editing tokens $A_0$, which are residually fused with $V$ via gating $g(A_0)$ to form auxiliary visual tokens $A = V + g(A_0)$; (3)~\emph {Continue (Phase-2 Generate)}: the LLM resumes decoding with $A$ in context to produce the final answer. \textbf {Right:} An illustrative geometry reasoning example where SCALER triggers \texttt {<auxiliary>} to synthesize the auxiliary diagram of $\triangle HCD$ and its altitude $HP$.\relax }{figure.caption.3}{main.pdf}}
\SCOLARExternalLabel{fig:method@cref}{{[figure][3][]3}{[1][2][]3}{}{}{main.pdf}}
\SCOLARExternalLabel{fig:training}{{4}{4}{\textbf {Overview of the SCALER Training Pipeline.} \textbf {Stage 1:} Detransformer pretraining via delta-feature reconstruction. \textbf {Stage 2:} Trigger learning via weighted NTP. \textbf {Stage 3:} Joint reasoning with teacher-forcing annealing. \textbf {RL:} ALPO with differentiable latent recomputation and outcome rewards.\relax }{figure.caption.4}{main.pdf}}
\SCOLARExternalLabel{fig:training@cref}{{[figure][4][]4}{[1][3][]4}{}{}{main.pdf}}
\SCOLARExternalLabel{sec:inference}{{3.1}{4}{\texorpdfstring {\hskip -1em.~}{}Overview}{subsection.3.1}{main.pdf}}
\SCOLARExternalLabel{sec:inference@cref}{{[subsection][1][3]3.1}{[1][3][]4}{}{}{main.pdf}}
\SCOLARExternalLabel{eq:inject}{{3}{4}{\texorpdfstring {\hskip -1em.~}{}Overview}{equation.3.3}{main.pdf}}
\SCOLARExternalLabel{eq:inject@cref}{{[equation][3][]3}{[1][4][]4}{}{}{main.pdf}}
\SCOLARExternalLabel{sec:sft_data}{{3.2}{4}{\texorpdfstring {\hskip -1em.~}{}Supervised Fine-Tuning (SFT)}{subsection.3.2}{main.pdf}}
\SCOLARExternalLabel{sec:sft_data@cref}{{[subsection][2][3]3.2}{[1][4][]4}{}{}{main.pdf}}
\SCOLARExternalLabel{tab:exp-main}{{1}{5}{\textbf {Performance on real-world perception and reasoning benchmarks.} The best-performing open-source model for each dataset is highlighted in \textbf {bold}, while the second-best is marked with an \underline {underline}.\relax }{table.caption.5}{main.pdf}}
\SCOLARExternalLabel{tab:exp-main@cref}{{[table][1][]1}{[1][4][]5}{}{}{main.pdf}}
\SCOLARExternalLabel{tab:exp-visualpuzzles}{{2}{6}{\textbf {Performance on VisualPuzzles (OOD).} Best open-source results are in \textbf {bold}, and second-best are \underline {underlined}.\relax }{table.caption.6}{main.pdf}}
\SCOLARExternalLabel{tab:exp-visualpuzzles@cref}{{[table][2][]2}{[1][6][]6}{}{}{main.pdf}}
\SCOLARExternalLabel{fig:filling}{{5}{7}{\textbf {Latent Length Scaling \& Meaningless Padding Experiments on (a) V*\,Bench, (b) MME-RealWorld-Lite, and (c) VisualPuzzles.} Solid lines: normal inference across latent lengths; dashed lines: replacing generated latents with meaningless padding; shaded regions: contribution of genuine latent semantics.\relax }{figure.caption.9}{main.pdf}}
\SCOLARExternalLabel{fig:filling@cref}{{[figure][5][]5}{[1][7][]7}{}{}{main.pdf}}
\SCOLARExternalLabel{sec:scaling_bottleneck}{{4.3}{7}{\texorpdfstring {\hskip -1em.~}{}Analysis of the Latent Scaling Bottleneck}{subsection.4.3}{main.pdf}}
\SCOLARExternalLabel{sec:scaling_bottleneck@cref}{{[subsection][3][4]4.3}{[1][7][]7}{}{}{main.pdf}}
\SCOLARExternalLabel{sec:padding_exp}{{4.4}{7}{\texorpdfstring {\hskip -1em.~}{}Latent Length Scaling and Meaningless Padding Experiments}{subsection.4.4}{main.pdf}}
\SCOLARExternalLabel{sec:padding_exp@cref}{{[subsection][4][4]4.4}{[1][7][]7}{}{}{main.pdf}}
\SCOLARExternalLabel{sec:novelty_exp}{{4.5}{8}{\texorpdfstring {\hskip -1em.~}{}Analysis of Step-wise Cosine Novelty and Latent Representation Saturation}{subsection.4.5}{main.pdf}}
\SCOLARExternalLabel{sec:novelty_exp@cref}{{[subsection][5][4]4.5}{[1][8][]8}{}{}{main.pdf}}
\SCOLARExternalLabel{tab:exp-ablation}{{3}{8}{\textbf {Ablation study.} Top block: inference-time interventions on SCALER-7B; bottom block: RL and SFT stage ablations relative to SCALER-SFT. Overall accuracy (\%) is reported.\relax }{table.caption.12}{main.pdf}}
\SCOLARExternalLabel{tab:exp-ablation@cref}{{[table][3][]3}{[1][8][]8}{}{}{main.pdf}}


==> xref_support.tex <==
% Import reference metadata only. This file never inputs the other document.
% Each entry point refreshes its own metadata after its .aux has been closed.
\makeatletter
\newcommand{\SCOLARExternalLabel}[2]{%
  \expandafter\gdef\csname r@#1\endcsname{#2}%
}
\newcommand{\SCOLARImportExternal}[1]{%
  \InputIfFileExists{xref_#1.tex}{}{}%
}
\newread\SCOLAR@refin
\newwrite\SCOLAR@refout
\long\def\SCOLAR@serialize#1#2#3#4#5#6\SCOLAR@stop{%
  \immediate\write\SCOLAR@refout{%
    \string\SCOLARExternalLabel{#1}{\unexpanded{{#2}{#3}{#4}{#5}}{\SCOLARDocument.pdf}}}%
}
\long\def\SCOLAR@checkline#1#2#3#4\SCOLAR@stop{%
  \ifx#1\newlabel
    \SCOLAR@serialize{#2}#3{}{}{}{}{}\SCOLAR@stop
  \fi
}
\def\SCOLAR@exportrefs{%
  \begingroup
  \openin\SCOLAR@refin=\jobname.aux\relax
  \ifeof\SCOLAR@refin\else
    \immediate\openout\SCOLAR@refout=xref_\SCOLARDocument.tex\relax
    \immediate\write\SCOLAR@refout{\@percentchar Generated labels from \SCOLARDocument.tex; no manuscript content.}%
    \loop\unless\ifeof\SCOLAR@refin
      \read\SCOLAR@refin to\SCOLAR@line
      \expandafter\SCOLAR@checkline\SCOLAR@line...\SCOLAR@stop
    \repeat
    \immediate\closeout\SCOLAR@refout
  \fi
  \closein\SCOLAR@refin
  \endgroup
}
\AddToHook{enddocument/afteraux}{\SCOLAR@exportrefs}
\makeatother

